ExoGAN: Retrieving Exoplanetary Atmospheres Using Deep Convolutional Generative Adversarial Networks

Atmospheric retrievals on exoplanets usually involve computationally intensive Bayesian sampling methods. Large parameter spaces and increasingly complex atmospheric models create a computational bottleneck forcing a trade-off between statistical sampling accuracy and model complexity. It is especially true for upcoming JWST and ARIEL observations. We introduce ExoGAN, the Exoplanet Generative Adversarial Network, a new deep learning algorithm able to recognise molecular features, atmospheric trace-gas abundances and planetary parameters using unsupervised learning. Once trained, ExoGAN is widely applicable to a large number of instruments and planetary types. The ExoGAN retrievals constitute a significant speed improvement over traditional retrievals and can be used either as a final atmospheric analysis or provide prior constraints to subsequent retrieval.

==> exogan <==
%% Created using Papers on Tue, 7 Jun 2018.
%% http://papersapp.com/papers/

@ARTICLE{2018AJ....155..156T,
   author = {{Tsiaras}, A. and {Waldmann}, I.~P. and {Zingales}, T. and {Rocchetto}, M. and 
	{Morello}, G. and {Damiano}, M. and {Karpouzas}, K. and {Tinetti}, G. and 
	{McKemmish}, L.~K. and {Tennyson}, J. and {Yurchenko}, S.~N.
	},
    title = "{A Population Study of Gaseous Exoplanets}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1704.05413},
 primaryClass = "astro-ph.EP",
 keywords = {methods: data analysis, methods: statistical, planets and satellites: atmospheres },
     year = 2018,
    month = apr,
   volume = 155,
      eid = {156},
    pages = {156},
      doi = {10.3847/1538-3881/aaaf75},
   adsurl = {http://adsabs.harvard.edu/abs/2018AJ....155..156T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{2041-8205-850-2-L32,
  author={Kyle B. Sheppard and Avi M. Mandell and Patrick Tamburo and Siddharth Gandhi and Arazi Pinhas and Nikku
Madhusudhan and Drake Deming},
  title={Evidence for a Dayside Thermal Inversion and High Metallicity for the Hot Jupiter WASP-18b},
  journal={The Astrophysical Journal Letters},
  volume={850},
  number={2},
  pages={L32},
  url={http://stacks.iop.org/2041-8205/850/i=2/a=L32},
  year={2017},
  abstract={We find evidence for a strong thermal inversion in the dayside atmosphere of the highly irradiated hot Jupiter WASP-18b ( ##IMG## [http://ej.iop.org/images/2041-8205/850/2/L32/apjlaa9ae9ieqn1.gif] {${T}_{\mathrm{eq}}=2411\,{\rm{K}}$} , ##IMG## [http://ej.iop.org/images/2041-8205/850/2/L32/apjlaa9ae9ieqn2.gif] {$M=10.3\,{M}_{J}$} ) based on emission spectroscopy from Hubble Space Telescope secondary eclipse observations and Spitzer eclipse photometry. We demonstrate a lack of water vapor in either absorption or emission at 1.4 Œº m. However, we infer emission at 4.5 Œº m and absorption at 1.6 Œº m that we attribute to CO, as well as a non-detection of all other relevant species (e.g., TiO, VO). The most probable atmospheric retrieval solution indicates a C/O ratio of 1 and a high metallicity ( ##IMG## [http://ej.iop.org/images/2041-8205/850/2/L32/apjlaa9ae9ieqn3.gif] {${\rm{C}}/{\rm{H}}={283}_{-138}^{+395}\times $} solar). The derived composition and T/P profile suggest that WASP-18b is the first example of both a planet with a non-oxide driven thermal inversion and a planet with an atmospheric metallicity inconsistent with that predicted for Jupiter-mass planets at ##IMG## [http://ej.iop.org/images/2041-8205/850/2/L32/apjlaa9ae9ieqn4.gif] {$\gt 2\sigma $} . Future observations are necessary to confirm the unusual planetary properties implied by these results.}
}

@ARTICLE{2018Natur.557...68S,
       author = {{Spake}, J.~J. and {Sing}, D.~K. and {Evans}, T.~M. and
        {Oklop{\v{c}}i{\'c}}, A. and {Bourrier}, V. and {Kreidberg}, L.
        and {Rackham}, B.~V. and {Irwin}, J. and {Ehrenreich}, D. and
        {Wyttenbach}, A. and {Wakeford}, H.~R. and {Zhou}, Y. and
        {Chubb}, K.~L. and {Nikolov}, N. and {Goyal}, J.~M. and {Henry},
        G.~W. and {Williamson}, M.~H. and {Blumenthal}, S. and
        {Anderson}, D.~R. and {Hellier}, C. and {Charbonneau}, D. and
        {Udry}, S. and {Madhusudhan}, N.},
        title = "{Helium in the eroding atmosphere of an exoplanet}",
      journal = {\nat},
     keywords = {Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = May,
       volume = {557},
        pages = {68-70},
          doi = {10.1038/s41586-018-0067-5},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2018Natur.557...68S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2018arXiv180500029K,
   author = {{Kreidberg}, L. and {Line}, M.~R. and {Parmentier}, V. and {Stevenson}, K.~B. and 
	{Louden}, T. and {Bonnefoy}, M. and {Faherty}, J.~K. and {Henry}, G.~W. and 
	{Williamson}, M.~H. and {Stassun}, K. and {Bean}, J.~L. and 
	{Fortney}, J.~J. and {Showman}, A.~P. and {D{\'e}sert}, J.-M. and 
	{Arcangeli}, J.},
    title = "{Global Climate and Atmospheric Composition of the Ultra-Hot Jupiter WASP-103b from HST and Spitzer Phase Curve Observations}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1805.00029},
 primaryClass = "astro-ph.EP",
 keywords = {Astrophysics - Earth and Planetary Astrophysics},
     year = 2018,
    month = apr,
   adsurl = {http://adsabs.harvard.edu/abs/2018arXiv180500029K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018AJ....155...55B,
   author = {{Bruno}, G. and {Lewis}, N.~K. and {Stevenson}, K.~B. and {Filippazzo}, J. and 
	{Hill}, M. and {Fraine}, J.~D. and {Wakeford}, H.~R. and {Deming}, D. and 
	{Kilpatrick}, B. and {Line}, M.~R. and {Morley}, C.~V. and {Collins}, K.~A. and 
	{Conti}, D.~M. and {Garlitz}, J. and {Rodriguez}, J.~E.},
    title = "{A Comparative Study of WASP-67 b and HAT-P-38 b from WFC3 Data}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1712.03384},
 primaryClass = "astro-ph.EP",
 keywords = {planets and satellites: atmospheres, planets and satellites: gaseous planets, planets and satellites: individual: WASP-67 b, HAT-P-38 b, techniques: spectroscopic },
     year = 2018,
    month = feb,
   volume = 155,
      eid = {55},
    pages = {55},
      doi = {10.3847/1538-3881/aaa0c7},
   adsurl = {http://adsabs.harvard.edu/abs/2018AJ....155...55B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018arXiv180500424M,
   author = {{Mansfield}, M. and {Bean}, J.~L. and {Line}, M.~R. and {Parmentier}, V. and 
	{Kreidberg}, L. and {Desert}, J.-M. and {Fortney}, J.~J. and 
	{Stevenson}, K.~B. and {Arcangeli}, J. and {Dragomir}, D.},
    title = "{A HST/WFC3 Thermal Emission Spectrum of the Hot Jupiter HAT-P-7b}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1805.00424},
 primaryClass = "astro-ph.EP",
 keywords = {Astrophysics - Earth and Planetary Astrophysics},
     year = 2018,
    month = may,
   adsurl = {http://adsabs.harvard.edu/abs/2018arXiv180500424M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2017arXiv170604987R,
   author = {{Rosca}, M. and {Lakshminarayanan}, B. and {Warde-Farley}, D. and 
	{Mohamed}, S.},
    title = "{Variational Approaches for Auto-Encoding Generative Adversarial Networks}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1706.04987},
 primaryClass = "stat.ML",
 keywords = {Statistics - Machine Learning, Computer Science - Learning},
     year = 2017,
    month = jun,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170604987R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@incollection{NIPS2016_6158,
title = {Generating Images with Perceptual Similarity Metrics based on Deep Networks},
author = {Dosovitskiy, Alexey and Brox, Thomas},
booktitle = {Advances in Neural Information Processing Systems 29},
editor = {D. D. Lee and M. Sugiyama and U. V. Luxburg and I. Guyon and R. Garnett},
pages = {658--666},
year = {2016},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/6158-generating-images-with-perceptual-similarity-metrics-based-on-deep-networks.pdf}
}

@ARTICLE{2017arXiv170402304U,
   author = {{Ulyanov}, D. and {Vedaldi}, A. and {Lempitsky}, V.},
    title = "{It Takes (Only) Two: Adversarial Generator-Encoder Networks}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1704.02304},
 primaryClass = "cs.CV",
 keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Learning, Statistics - Machine Learning},
     year = 2017,
    month = apr,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170402304U},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015arXiv151105644M,
   author = {{Makhzani}, A. and {Shlens}, J. and {Jaitly}, N. and {Goodfellow}, I. and 
	{Frey}, B.},
    title = "{Adversarial Autoencoders}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1511.05644},
 primaryClass = "cs.LG",
 keywords = {Computer Science - Learning},
     year = 2015,
    month = nov,
   adsurl = {http://adsabs.harvard.edu/abs/2015arXiv151105644M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@article{2009ApJ...707...24M,
author = {Madhusudhan, N and Seager, S},
title = {{A Temperature and Abundance Retrieval Method for Exoplanet Atmospheres}},
journal = {The Astrophysical Journal},
year = {2009},
volume = {707},
number = {1},
pages = {24--39},
month = dec
}

@MISC{2016ascl.soft08004C,
       author = {{Cubillos}, Patricio and {Blecic}, Jasmina and {Harrington}, Joseph and
        {Rojo}, Patricio and {Lust}, Nate and {Bowman}, Oliver and
        {Stemm}, Madison and {Foster}, Andrew and {Loredo}, Thomas J.
        and {Fortney}, Jonathan and {Madhusudhan}, Nikku},
        title = "{BART: Bayesian Atmospheric Radiative Transfer fitting code}",
     keywords = {Software},
 howpublished = {Astrophysics Source Code Library},
         year = 2016,
        month = Aug,
          eid = {ascl:1608.004},
        pages = {ascl:1608.004},
archivePrefix = {ascl},
       eprint = {1608.004},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2016ascl.soft08004C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{2008JQSRT.109.1136I,
author = {Irwin, P G J and Teanby, N A and De Kok, R and Fletcher, L N and Howett, C J A and Tsang, C C C and Wilson, C F and Calcutt, S B and Nixon, C A and Parrish, P D},
title = {{The NEMESIS planetary atmosphere radiative transfer and retrieval tool}},
journal = {Journal of Quantitative Spectroscopy {\&} Radiative Transfer},
year = {2008},
volume = {109},
number = {6},
pages = {1136--1150},
month = apr
}

@ARTICLE{2017AJ....154...91L,
       author = {{Lavie}, Baptiste and {Mendon{\c{c}}a}, Jo{\~a}o M. and {Mordasini},
        Christoph and {Malik}, Matej and {Bonnefoy}, Micka{\"e}l and
        {Demory}, Brice-Olivier and {Oreshenko}, Maria and {Grimm},
        Simon L. and {Ehrenreich}, David and {Heng}, Kevin},
        title = "{HELIOS-RETRIEVAL: An Open-source, Nested Sampling Atmospheric Retrieval
        Code; Application to the HR 8799 Exoplanets and Inferred
        Constraints for Planet Formation}",
      journal = {\aj},
     keywords = {methods: statistical, planets and satellites: atmospheres, planets and
        satellites: composition, planets and satellites: formation,
        planets and satellites: gaseous planets, planets and satellites:
        individual: HR 8799, Astrophysics - Earth and Planetary
        Astrophysics, Physics - Atmospheric and Oceanic Physics},
         year = 2017,
        month = Sep,
       volume = {154},
          eid = {91},
        pages = {91},
          doi = {10.3847/1538-3881/aa7ed8},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2017AJ....154...91L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{2013ApJ...775..137L,
author = {Line, Michael R and Wolf, Aaron S and Zhang, Xi and Knutson, Heather and Kammer, Joshua A and Ellison, Elias and Deroo, Pieter and Crisp, Dave and Yung, Yuk L},
title = {{A Systematic Retrieval Analysis of Secondary Eclipse Spectra. I. A Comparison of Atmospheric Retrieval Techniques}},
journal = {The Astrophysical Journal},
year = {2013},
volume = {775},
number = {2},
pages = {137},
month = oct,
annote = {27 pages, 13 figures}
}


@article{Benneke:2013vx,
author = {Benneke, Bj{\"o}rn and Seager, Sara},
title = {{How to Distinguish between Cloudy Mini-Neptunes and Water/Volatile-dominated Super-Earths}},
journal = {APJ},
year = {2013},
volume = {778},
number = {2},
pages = {153},
month = dec
}

@article{doi:10.1093/mnras/stx2748,
author = {Gandhi, Siddharth and Madhusudhan, Nikku},
title = {Retrieval of exoplanet emission spectra with HyDRA},
journal = {Monthly Notices of the Royal Astronomical Society},
volume = {474},
number = {1},
pages = {271-288},
year = {2018},
doi = {10.1093/mnras/stx2748},
URL = {http://dx.doi.org/10.1093/mnras/stx2748},
eprint = {/oup/backfile/content_public/journal/mnras/474/1/10.1093_mnras_stx2748/2/stx2748.pdf}
}


@ARTICLE{2018MNRAS.477.2513S,
   author = {{Stark}, D. and {Launet}, B. and {Schawinski}, K. and {Zhang}, C. and 
	{Koss}, M. and {Turp}, M.~D. and {Sartori}, L.~F. and {Zhang}, H. and 
	{Chen}, Y. and {Weigel}, A.~K.},
    title = "{PSFGAN: a generative adversarial network system for separating quasar point sources and host galaxy light}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1803.08925},
 keywords = {methods: data analysis, techniques: image processing, quasars: general},
     year = 2018,
    month = jun,
   volume = 477,
    pages = {2513-2527},
      doi = {10.1093/mnras/sty764},
   adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.477.2513S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{doi:10.1093/mnrasl/slx008,
author = {Schawinski, Kevin and Zhang, Ce and Zhang, Hantian and Fowler, Lucas and Santhanam, Gokula Krishnan},
title = {Generative adversarial networks recover features in astrophysical images of galaxies beyond the deconvolution limit},
journal = {Monthly Notices of the Royal Astronomical Society: Letters},
volume = {467},
number = {1},
pages = {L110-L114},
year = {2017},
doi = {10.1093/mnrasl/slx008},
URL = {http://dx.doi.org/10.1093/mnrasl/slx008},
eprint = {/oup/backfile/content_public/journal/mnrasl/467/1/10.1093_mnrasl_slx008/1/slx008.pdf}
}




@ARTICLE{2013arXiv1312.6114K,
   author = {{Kingma}, D.~P and {Welling}, M.},
    title = "{Auto-Encoding Variational Bayes}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1312.6114},
 primaryClass = "stat.ML",
 keywords = {Statistics - Machine Learning, Computer Science - Learning},
     year = 2013,
    month = dec,
   adsurl = {http://adsabs.harvard.edu/abs/2013arXiv1312.6114K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014arXiv1401.4082J,
   author = {{Jimenez Rezende}, D. and {Mohamed}, S. and {Wierstra}, D.},
    title = "{Stochastic Backpropagation and Approximate Inference in Deep Generative Models}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1401.4082},
 primaryClass = "stat.ML",
 keywords = {Statistics - Machine Learning, Computer Science - Artificial Intelligence, Computer Science - Learning, Statistics - Computation, Statistics - Methodology},
     year = 2014,
    month = jan,
   adsurl = {http://adsabs.harvard.edu/abs/2014arXiv1401.4082J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{Bengio:2009kb,
author = {Bengio, Yoshua},
title = {{Learning Deep Architectures for AI}},
publisher = {Now Publishers Inc},
year = {2009},
volume = {2}
}

@incollection{Rumelhart:1986:LIR:104279.104293,
 author = {Rumelhart, D. E. and Hinton, G. E. and Williams, R. J.},
 chapter = {Learning Internal Representations by Error Propagation},
 title = {Parallel Distributed Processing: Explorations in the Microstructure of Cognition, Vol. 1},
 editor = {Rumelhart, David E. and McClelland, James L. and PDP Research Group, CORPORATE},
 year = {1986},
 isbn = {0-262-68053-X},
 pages = {318--362},
 numpages = {45},
 url = {http://dl.acm.org/citation.cfm?id=104279.104293},
 acmid = {104293},
 publisher = {MIT Press},
 address = {Cambridge, MA, USA},
} 

@article{2008MNRAS.384..449F,
author = {Feroz, F and Hobson, M P},
title = {{Multimodal nested sampling: an efficient and robust alternative to Markov Chain Monte Carlo methods for astronomical data analyses}},
journal = {Monthly Notices of the Royal Astronomical Society},
year = {2008},
volume = {384},
number = {2},
pages = {449--463},
month = feb
}

@article{Feroz:2009jn,
author = {Feroz, Farhan and Gair, Jonathan R and Hobson, Michael P and Porter, Edward K},
title = {{Use of the MULTINEST algorithm for gravitational wave data analysis}},
journal = {Classical and Quantum Gravity},
year = {2009},
volume = {26},
number = {21},
pages = {215003},
month = oct
}

@article{2004AIPC..735..395S,
author = {Skilling, John},
title = {{Nested Sampling}},
journal = {Bayesian Inference and Maximum Entropy Methods in Science and Engineering: 24th International Workshop on Bayesian Inference and Maximum Entropy Methods in Science and Engineering held 25-30 July},
year = {2004},
volume = {735},
pages = {395--405},
month = nov
}

@article{gregory11,
author = {Gregory, P C},
title = {{Bayesian exoplanet tests of a new method for MCMC sampling in highly correlated model parameter spaces}},
journal = {MNRAS},
year = {2011},
volume = {410},
pages = {94--110}
}

@ARTICLE{2018MNRAS.474..478P,
       author = {{Pearson}, Kyle A. and {Palafox}, Leon and {Griffith}, Caitlin A.},
        title = "{Searching for exoplanets using artificial intelligence}",
      journal = {\mnras},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics,
        Astrophysics - Earth and Planetary Astrophysics},
         year = 2018,
        month = Feb,
       volume = {474},
        pages = {478-491},
          doi = {10.1093/mnras/stx2761},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2018MNRAS.474..478P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017MNRAS.465.3495K,
       author = {{Kipping}, David M. and {Lam}, Christopher},
        title = "{Transit clairvoyance: enhancing TESS follow-up using artificial neural
        networks}",
      journal = {\mnras},
     keywords = {methods: numerical, eclipses, planets and satellites: detection,
        planetary systems, Astrophysics - Instrumentation and Methods
        for Astrophysics, Astrophysics - Earth and Planetary
        Astrophysics},
         year = 2017,
        month = Mar,
       volume = {465},
        pages = {3495-3505},
          doi = {10.1093/mnras/stw2974},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2017MNRAS.465.3495K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016ApJ...833..120R,
       author = {{Rocchetto}, M. and {Waldmann}, I.~P. and {Venot}, O. and {Lagage}, P.
        -O. and {Tinetti}, G.},
        title = "{Exploring Biases of Atmospheric Retrievals in Simulated JWST
        Transmission Spectra of Hot Jupiters}",
      journal = {\apj},
     keywords = {methods: data analysis, methods: statistical, techniques: spectroscopic,
        Astrophysics - Earth and Planetary Astrophysics},
         year = 2016,
        month = Dec,
       volume = {833},
          eid = {120},
        pages = {120},
          doi = {10.3847/1538-4357/833/1/120},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2016ApJ...833..120R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2018AJ....155...94S,
   author = {{Shallue}, C.~J. and {Vanderburg}, A.},
    title = "{Identifying Exoplanets with Deep Learning: A Five-planet Resonant Chain around Kepler-80 and an Eighth Planet around Kepler-90}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1712.05044},
 primaryClass = "astro-ph.EP",
 keywords = {methods: data analysis, planets and satellites: detection, techniques: photometric },
     year = 2018,
    month = feb,
   volume = 155,
      eid = {94},
    pages = {94},
      doi = {10.3847/1538-3881/aa9e09},
   adsurl = {http://adsabs.harvard.edu/abs/2018AJ....155...94S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017ApJ...834...50B,
   author = {{Barstow}, J.~K. and {Aigrain}, S. and {Irwin}, P.~G.~J. and 
	{Sing}, D.~K.},
    title = "{A Consistent Retrieval Analysis of 10 Hot Jupiters Observed in Transmission}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1610.01841},
 primaryClass = "astro-ph.EP",
 keywords = {Methods: data analysis, planets and satellites: atmospheres, radiative transfer},
     year = 2017,
    month = jan,
   volume = 834,
      eid = {50},
    pages = {50},
      doi = {10.3847/1538-4357/834/1/50},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...834...50B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{2016SPIE.9904E..1XT,
       author = {{Tinetti}, G. and {Drossart}, P. and {Eccleston}, P. and {Hartogh}, P.
        and {Heske}, A. and {Leconte}, J. and {Micela}, G. and
        {Ollivier}, M. and {Pilbratt}, G. and {Puig}, L. and {Turrini},
        D. and {Vandenbussche}, B. and {Wolkenberg}, P. and {Pascale},
        E. and {Beaulieu}, J. -P. and {G{\"u}del}, M. and {Min}, M. and
        {Rataj}, M. and {Ray}, T. and {Ribas}, I. and {Barstow}, J. and
        {Bowles}, N. and {Coustenis}, A. and {Coud{\'e} du Foresto}, V.
        and {Decin}, L. and {Encrenaz}, T. and {Forget}, F. and
        {Friswell}, M. and {Griffin}, M. and {Lagage}, P.~O. and
        {Malaguti}, P. and {Moneti}, A. and {Morales}, J.~C. and {Pace},
        E. and {Rocchetto}, M. and {Sarkar}, S. and {Selsis}, F. and
        {Taylor}, W. and {Tennyson}, J. and {Venot}, O. and {Waldmann},
        I.~P. and {Wright}, G. and {Zingales}, T. and {Zapatero-Osorio},
        M.~R.},
        title = "{The science of ARIEL (Atmospheric Remote-sensing Infrared Exoplanet
        Large-survey)}",
    booktitle = {Space Telescopes and Instrumentation 2016: Optical, Infrared, and Millimeter Wave},
         year = 2016,
       volume = {9904},
        month = Jul,
          eid = {99041X},
        pages = {99041X},
          doi = {10.1117/12.2232370},
       adsurl = {https://ui.adsabs.harvard.edu/#abs/2016SPIE.9904E..1XT},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@Article{Gardner2006,
author="Gardner, Jonathan P.
and Mather, John C.
and Clampin, Mark
and Doyon, Rene
and Greenhouse, Matthew A.
and Hammel, Heidi B.
and Hutchings, John B.
and Jakobsen, Peter
and Lilly, Simon J.
and Long, Knox S.
and Lunine, Jonathan I.
and Mccaughrean, Mark J.
and Mountain, Matt
and Nella, John
and Rieke, George H.
and Rieke, Marcia J.
and Rix, Hans-Walter
and Smith, Eric P.
and Sonneborn, George
and Stiavelli, Massimo
and Stockman, H. S.
and Windhorst, Rogier A.
and Wright, Gillian S.",
title="The James Webb Space Telescope",
journal="Space Science Reviews",
year="2006",
month="Apr",
day="01",
volume="123",
number="4",
pages="485--606",
abstract="The James Webb Space Telescope (JWST) is a large (6.6 m), cold (<50 K), infrared (IR)-optimized space observatory that will be launched early in the next decade into orbit around the second Earth--Sun Lagrange point. The observatory will have four instruments: a near-IR camera, a near-IR multiobject spectrograph, and a tunable filter imager will cover the wavelength range, 0.6 < ; < 5.0 $\mu$ m, while the mid-IR instrument will do both imaging and spectroscopy from 5.0 < ; < 29  $\mu$ m.",
issn="1572-9672",
doi="10.1007/s11214-006-8315-7",
url="https://doi.org/10.1007/s11214-006-8315-7"
}


@ARTICLE{2014arXiv1412.6980K,
   author = {{Kingma}, D.~P. and {Ba}, J.},
    title = "{Adam: A Method for Stochastic Optimization}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1412.6980},
 primaryClass = "cs.LG",
 keywords = {Computer Science - Learning},
     year = 2014,
    month = dec,
   adsurl = {http://adsabs.harvard.edu/abs/2014arXiv1412.6980K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2016ApJ...820..107W,
   author = {{Waldmann}, I.~P.},
    title = "{Dreaming of Atmospheres}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1511.08339},
 primaryClass = "astro-ph.EP",
 keywords = {methods: data analysis, methods: statistical, radiative transfer, techniques: spectroscopic},
     year = 2016,
    month = apr,
   volume = 820,
      eid = {107},
    pages = {107},
      doi = {10.3847/0004-637X/820/2/107},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...820..107W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018arXiv180109070R,
   author = {{Rodriguez}, A.~C and {Kacprzak}, T. and {Lucchi}, A. and {Amara}, A. and 
	{Sgier}, R. and {Fluri}, J. and {Hofmann}, T. and {R{\'e}fr{\'e}gier}, A.
	},
    title = "{Fast Cosmic Web Simulations with Generative Adversarial Networks}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1801.09070},
 keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, Statistics - Machine Learning},
     year = 2018,
    month = jan,
   adsurl = {http://adsabs.harvard.edu/abs/2018arXiv180109070R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015arXiv150605751D,
   author = {{Denton}, E. and {Chintala}, S. and {Szlam}, A. and {Fergus}, R.
	},
    title = "{Deep Generative Image Models using a Laplacian Pyramid of Adversarial Networks}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1506.05751},
 primaryClass = "cs.CV",
 keywords = {Computer Science - Computer Vision and Pattern Recognition},
     year = 2015,
    month = jun,
   adsurl = {http://adsabs.harvard.edu/abs/2015arXiv150605751D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2017arXiv170104862A,
   author = {{Arjovsky}, M. and {Bottou}, L.},
    title = "{Towards Principled Methods for Training Generative Adversarial Networks}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1701.04862},
 primaryClass = "stat.ML",
 keywords = {Statistics - Machine Learning, Computer Science - Learning},
     year = 2017,
    month = jan,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170104862A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2018ISPM...35...53C,
   author = {{Creswell}, A. and {White}, T. and {Dumoulin}, V. and {Arulkumaran}, K. and 
	{Sengupta}, B. and {Bharath}, A.~A.},
    title = "{Generative Adversarial Networks: An Overview}",
  journal = {IEEE Signal Processing Magazine},
archivePrefix = "arXiv",
   eprint = {1710.07035},
 primaryClass = "cs.CV",
     year = 2018,
    month = jan,
   volume = 35,
    pages = {53-65},
      doi = {10.1109/MSP.2017.2765202},
   adsurl = {http://adsabs.harvard.edu/abs/2018ISPM...35...53C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014arXiv1406.2661G,
   author = {{Goodfellow}, I.~J. and {Pouget-Abadie}, J. and {Mirza}, M. and 
	{Xu}, B. and {Warde-Farley}, D. and {Ozair}, S. and {Courville}, A. and 
	{Bengio}, Y.},
    title = "{Generative Adversarial Networks}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1406.2661},
 primaryClass = "stat.ML",
 keywords = {Statistics - Machine Learning, Computer Science - Learning},
     year = 2014,
    month = jun,
   adsurl = {http://adsabs.harvard.edu/abs/2014arXiv1406.2661G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017arXiv170509558S,
   author = {{Saatchi}, Y. and {Wilson}, A.~G.},
    title = "{Bayesian GAN}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1705.09558},
 primaryClass = "stat.ML",
 keywords = {Statistics - Machine Learning, Computer Science - Artificial Intelligence, Computer Science - Computer Vision and Pattern Recognition, Computer Science - Learning},
     year = 2017,
    month = may,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170509558S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017arXiv170100160G,
   author = {{Goodfellow}, I.},
    title = "{NIPS 2016 Tutorial: Generative Adversarial Networks}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1701.00160},
 primaryClass = "cs.LG",
 keywords = {Computer Science - Learning},
     year = 2017,
    month = dec,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170100160G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2016arXiv161102163M,
   author = {{Metz}, L. and {Poole}, B. and {Pfau}, D. and {Sohl-Dickstein}, J.
	},
    title = "{Unrolled Generative Adversarial Networks}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1611.02163},
 primaryClass = "cs.LG",
 keywords = {Computer Science - Learning, Statistics - Machine Learning},
     year = 2016,
    month = nov,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv161102163M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2016arXiv160707539Y,
   author = {{Yeh}, R.~A. and {Chen}, C. and {Yian Lim}, T. and {Schwing}, A.~G. and 
	{Hasegawa-Johnson}, M. and {Do}, M.~N.},
    title = "{Semantic Image Inpainting with Deep Generative Models}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1607.07539},
 primaryClass = "cs.CV",
 keywords = {Computer Science - Computer Vision and Pattern Recognition},
     year = 2016,
    month = jul,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160707539Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@misc{amos2016image,
    title        = {{Image Completion with Deep Learning in TensorFlow}},
    author       = {Amos, Brandon},
    howpublished = {\url{http://bamos.github.io/2016/08/09/deep-completion}},
    year		 = {2016},
    note         = {Accessed: 12/05/2018}
}

@ARTICLE{2016arXiv160407379P,
   author = {{Pathak}, D. and {Krahenbuhl}, P. and {Donahue}, J. and {Darrell}, T. and 
	{Efros}, A.~A.},
    title = "{Context Encoders: Feature Learning by Inpainting}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1604.07379},
 primaryClass = "cs.CV",
 keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Artificial Intelligence, Computer Science - Graphics, Computer Science - Learning},
     year = 2016,
    month = apr,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160407379P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2016arXiv160908144W,
   author = {{Wu}, Y. and {Schuster}, M. and {Chen}, Z. and {Le}, Q.~V. and 
	{Norouzi}, M. and {Macherey}, W. and {Krikun}, M. and {Cao}, Y. and 
	{Gao}, Q. and {Macherey}, K. and {Klingner}, J. and {Shah}, A. and 
	{Johnson}, M. and {Liu}, X. and {Kaiser}, {\L}. and {Gouws}, S. and 
	{Kato}, Y. and {Kudo}, T. and {Kazawa}, H. and {Stevens}, K. and 
	{Kurian}, G. and {Patil}, N. and {Wang}, W. and {Young}, C. and 
	{Smith}, J. and {Riesa}, J. and {Rudnick}, A. and {Vinyals}, O. and 
	{Corrado}, G. and {Hughes}, M. and {Dean}, J.},
    title = "{Google's Neural Machine Translation System: Bridging the Gap between Human and Machine Translation}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1609.08144},
 primaryClass = "cs.CL",
 keywords = {Computer Science - Computation and Language, Computer Science - Artificial Intelligence, Computer Science - Learning},
     year = 2016,
    month = sep,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160908144W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2016arXiv160203220L,
   author = {{Lamb}, A. and {Dumoulin}, V. and {Courville}, A.},
    title = "{Discriminative Regularization for Generative Models}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1602.03220},
 primaryClass = "stat.ML",
 keywords = {Statistics - Machine Learning, Computer Science - Learning},
     year = 2016,
    month = feb,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160203220L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2016arXiv160603498S,
   author = {{Salimans}, T. and {Goodfellow}, I. and {Zaremba}, W. and {Cheung}, V. and 
	{Radford}, A. and {Chen}, X.},
    title = "{Improved Techniques for Training GANs}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1606.03498},
 primaryClass = "cs.LG",
 keywords = {Computer Science - Learning, Computer Science - Computer Vision and Pattern Recognition, Computer Science - Neural and Evolutionary Computing},
     year = 2016,
    month = jun,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160603498S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{corner,
    Author = {Daniel Foreman-Mackey},
    Doi = {10.21105/joss.00024},
    Title = {corner.py: Scatterplot matrices in Python},
    Journal = {The Journal of Open Source Software},
    Year = 2016,
    Volume = 24,
    Url = {http://dx.doi.org/10.5281/zenodo.45906}
}

@ARTICLE{2015arXiv151106434R,
   author = {{Radford}, A. and {Metz}, L. and {Chintala}, S.},
    title = "{Unsupervised Representation Learning with Deep Convolutional Generative Adversarial Networks}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1511.06434},
 primaryClass = "cs.LG",
 keywords = {Computer Science - Learning, Computer Science - Computer Vision and Pattern Recognition},
     year = 2015,
    month = nov,
   adsurl = {http://adsabs.harvard.edu/abs/2015arXiv151106434R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015ApJ...802..107W,
	author = {{Waldmann}, I.~P. and {Tinetti}, G. and {Rocchetto}, M. and 
	{Barton}, E.~J. and {Yurchenko}, S.~N. and {Tennyson}, J.},
	title = "{Tau-REx I: A Next Generation Retrieval Code for Exoplanetary Atmospheres}",
	journal = {\apj},
	archivePrefix = "arXiv",
	eprint = {1409.2312},
	primaryClass = "astro-ph.EP",
	keywords = {methods: data analysis, methods: statistical, radiative transfer, techniques: spectroscopic},
	year = 2015,
	month = apr,
	volume = 802,
	eid = {107},
	pages = {107},
	doi = {10.1088/0004-637X/802/2/107},
	adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...802..107W},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008ApJ...677.1324T,
   author = {{Torres}, G. and {Winn}, J.~N. and {Holman}, M.~J.},
    title = "{Improved Parameters for Extrasolar Transiting Planets}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0801.1841},
 keywords = {methods: data analysis, planetary systems, stars: abundances, stars: fundamental parameters, techniques: spectroscopic},
     year = 2008,
    month = apr,
   volume = 677,
    pages = {1324-1342},
      doi = {10.1086/529429},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...677.1324T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015arXiv150500853X,
   author = {{Xu}, B. and {Wang}, N. and {Chen}, T. and {Li}, M.},
    title = "{Empirical Evaluation of Rectified Activations in Convolutional Network}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1505.00853},
 primaryClass = "cs.LG",
 keywords = {Computer Science - Learning, Computer Science - Computer Vision and Pattern Recognition, Statistics - Machine Learning},
     year = 2015,
    month = may,
   adsurl = {http://adsabs.harvard.edu/abs/2015arXiv150500853X},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{Goodfellow-et-al-2016,
    title={Deep Learning},
    author={Ian Goodfellow and Yoshua Bengio and Aaron Courville},
    publisher={MIT Press},
    note={\url{http://www.deeplearningbook.org}},
    year={2016}
}

@ARTICLE{2006ApJ...646..505B,
   author = {{Butler}, R.~P. and {Wright}, J.~T. and {Marcy}, G.~W. and {Fischer}, D.~A. and 
	{Vogt}, S.~S. and {Tinney}, C.~G. and {Jones}, H.~R.~A. and 
	{Carter}, B.~D. and {Johnson}, J.~A. and {McCarthy}, C. and 
	{Penny}, A.~J.},
    title = "{Catalog of Nearby Exoplanets}",
  journal = {\apj},
   eprint = {astro-ph/0607493},
 keywords = {Stars: Planetary Systems, Stars: Activity, Stars: Chromospheres},
     year = 2006,
    month = jul,
   volume = 646,
    pages = {505-522},
      doi = {10.1086/504701},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...646..505B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2015ApJ...813...13W,
	author = {{Waldmann}, I.~P. and {Rocchetto}, M. and {Tinetti}, G. and 
	{Barton}, E.~J. and {Yurchenko}, S.~N. and {Tennyson}, J.},
	title = "{Tau-REx II: Retrieval of Emission Spectra}",
	journal = {\apj},
	archivePrefix = "arXiv",
	eprint = {1508.07591},
	primaryClass = "astro-ph.EP",
	keywords = {methods: data analysis, methods: statistical, radiative transfer, techniques: spectroscopic},
	year = 2015,
	month = nov,
	volume = 813,
	eid = {13},
	pages = {13},
	doi = {10.1088/0004-637X/813/1/13},
	adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...813...13W},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018AJ....155..156T,
   author = {{Tsiaras}, A. and {Waldmann}, I.~P. and {Zingales}, T. and {Rocchetto}, M. and 
	{Morello}, G. and {Damiano}, M. and {Karpouzas}, K. and {Tinetti}, G. and 
	{McKemmish}, L.~K. and {Tennyson}, J. and {Yurchenko}, S.~N.
	},
    title = "{A Population Study of Gaseous Exoplanets}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1704.05413},
 primaryClass = "astro-ph.EP",
 keywords = {methods: data analysis, methods: statistical, planets and satellites: atmospheres },
     year = 2018,
    month = apr,
   volume = 155,
      eid = {156},
    pages = {156},
      doi = {10.3847/1538-3881/aaaf75},
   adsurl = {http://adsabs.harvard.edu/abs/2018AJ....155..156T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{corner,
    Author = {Daniel Foreman-Mackey},
    Doi = {10.21105/joss.00024},
    Title = {corner.py: Scatterplot matrices in Python},
    Journal = {The Journal of Open Source Software},
    Year = 2016,
    Volume = 24,
    Url = {http://dx.doi.org/10.5281/zenodo.45906}
}

@ARTICLE{2012A&A...546A..43V,
   author = {{Venot}, O. and {H{\'e}brard}, E. and {Ag{\'u}ndez}, M. and 
	{Dobrijevic}, M. and {Selsis}, F. and {Hersant}, F. and {Iro}, N. and 
	{Bounaceur}, R.},
    title = "{A chemical model for the atmosphere of hot Jupiters}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1208.0560},
 primaryClass = "astro-ph.EP",
 keywords = {astrochemistry, planets and satellites: atmospheres, planets and satellites: individual: HD 209458b, planets and satellites: individual: HD 189733b, planetary systems},
     year = 2012,
    month = oct,
   volume = 546,
      eid = {A43},
    pages = {A43},
      doi = {10.1051/0004-6361/201219310},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...546A..43V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



